Measurement of indirect $CP$ asymmetries in $D^0\rightarrow K^-K^+$ and $D^0\rightarrow \pi^-\pi^+$ decays using semileptonic $B$ decays

Time-dependent $CP$ asymmetries in the decay rates of the singly Cabibbo-suppressed decays $D^0\rightarrow K^-K^+$ and $D^0\rightarrow \pi^-\pi^+$ are measured in $pp$ collision data corresponding to an integrated luminosity of 3.0 fb$^{-1}$ collected by the LHCb experiment. The $D^0$ mesons are produced in semileptonic $b$-hadron decays, where the charge of the accompanying muon is used to determine the initial state as $D^0$ or $\bar{D}^0$. The asymmetries in effective lifetimes between $D^0$ and $\bar{D}^0$ decays, which are sensitive to indirect $CP$ violation, are determined to be \begin{align*} A_{\Gamma}(K^-K^+) = (-0.134 \pm 0.077 \; {}^{+0.026}_{-0.034})\% \, A_{\Gamma}(\pi^-\pi^+) = (-0.092\pm 0.145 \; {}^{+0.025}_{-0.033})\% \, \end{align*} where the first uncertainties are statistical and the second systematic. This result is in agreement with previous measurements and with the hypothesis of no indirect $CP$ violation in $D^0$ decays.

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 18784 2012-04-30 14:45:53Z uegede $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\bf LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}

